Logic Constrained Pointer Networks for Interpretable Textual Similarity

Systematically discovering semantic relationships in text is an important and extensively studied area in Natural Language Processing, with various tasks such as entailment, semantic similarity, etc. Decomposability of sentence-level scores via subsequence alignments has been proposed as a way to make models more interpretable. We study the problem of aligning components of sentences leading to an interpretable model for semantic textual similarity. In this paper, we introduce a novel pointer network based model with a sentinel gating function to align constituent chunks, which are represented using BERT. We improve this base model with a loss function to equally penalize misalignments in both sentences, ensuring the alignments are bidirectional. Finally, to guide the network with structured external knowledge, we introduce first-order logic constraints based on ConceptNet and syntactic knowledge. The model achieves an F1 score of 97.73 and 96.32 on the benchmark SemEval datasets for the chunk alignment task, showing large improvements over the existing solutions. Source code is available at https://github.com/manishb89/interpretable_sentence_similarity

==> 2-problem.tex <==
\section{Problem Definition}
The problem of interpretable semantic textual similarity is to provide an interpretation or explanation of semantic similarity between two texts (usually sentences). We consider chunking to be a preprocessing step and assume that the sentences are already chunked. Not all chunks in one sentence are aligned to a chunk in the other sentence. This is well motivated because sentences have varying degrees of similarity and similarity is proportional to number of aligned chunks. We consider these non-aligned chunks to be aligned to special empty chunk. Figure \ref{fig:alignment_example} provides an example to illustrate the problem.
%Formally, let $\mathbf{x}=(x_1, x_2,\ldots, x_n)$ and $\mathbf{y}=(y_1,y_2,\ldots, y_m)$ be two sentences, where $x_i$ (and $y_j$) are chunks (contiguous words) in $\mathbf{x}$ and $\mathbf{y}$, respectively. 

%The problem of iSTS is to then predict an alignment between chunks $z_{i,j}\in\{0,1\}$ indicating if $x_i$ and $y_j$ are aligned along with a score for alignment which indicates how strongly the two chunks are aligned. We consider a supervised setting in which the ground truth alignment $a_{i,j}\in\{0,1\}$ is specified in the training data. The score for alignment is an number between $1$ to $5$ with $5$ meaning very strongly aligned. 

\begin{figure}[!htb]
    \centering
    %\resizebox{\linewidth}{7cm} {
    \includegraphics[width=\linewidth, keepaspectratio]{Interpretable_sim_golden_example.png}
    %}
    \caption{Interpretable sentence similarity defined as alignments between chunks (indicated by connecting lines) of the two sentences. An unaligned chunk is considered aligned to special `not aligned' chunk (denoted by $\phi$ in paper).}
    \label{fig:alignment_example}
%\vspace{-6mm}
\end{figure}
%\fxnote{Provide an example from semeval dataset:Subhadeep, Example 70 from test set, example 76 from test set}
